Impact Of Magnetic Fields On Molecular Cloud Formation & Evolution

We use magnetohydrodynamical simulations of converging flows to investigate the process of molecular cloud formation and evolution out of the magnetised ISM. Here, we investigate whether the observed subcritical HI clouds can become supercritical and hence allow the formation of stars within them. To do so, we vary the turbulent Mach number of the flows, as well as the initial magnetic field strength. We show that dense cores are able to build up under all conditions, but that star formation in these cores is either heavily delayed or completely suppressed if the initial field strength is B>3 microGauss. To probe the effect of magnetic diffusion, we introduce a tilting angle between the flows and the uniform background magnetic field, which mimics non--ideal MHD effects. Even with highly inclined flows, the formed cores are devoid of star formation, because no magnetically supercritical regions are build up. Hence we conclude, that the problem of how supercritical cloud cores are generated still persists.

==> journals.tex <==
%% journal abbreviations (from aastex.cls)

\def\jnl@style#1{{\rmfamily#1}}%
\def\jref@jnl#1{{\jnl@style#1}}%

\newcommand\aj{\jref@jnl{AJ}}%
          % Astronomical Journal
\newcommand\araa{\jref@jnl{ARA\&A}}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{\jref@jnl{ApJ}}%
          % Astrophysical Journal
\newcommand\apjl{\jref@jnl{ApJ}}%
          % Astrophysical Journal, Letters
\newcommand\apjs{\jref@jnl{ApJS}}%
          % Astrophysical Journal, Supplement
\newcommand\ao{\jref@jnl{Appl.~Opt.}}%
          % Applied Optics
\newcommand\apss{\jref@jnl{Ap\&SS}}%
          % Astrophysics and Space Science
\newcommand\aap{\jref@jnl{A\&A}}%
          % Astronomy and Astrophysics
\newcommand\aapr{\jref@jnl{A\&A~Rev.}}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{\jref@jnl{A\&AS}}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{\jref@jnl{AZh}}%
          % Astronomicheskii Zhurnal
\newcommand\baas{\jref@jnl{BAAS}}%
          % Bulletin of the AAS
\newcommand\jrasc{\jref@jnl{JRASC}}%
          % Journal of the RAS of Canada
\newcommand\memras{\jref@jnl{MmRAS}}%
          % Memoirs of the RAS
\newcommand\mnras{\jref@jnl{MNRAS}}%
          % Monthly Notices of the RAS
\newcommand\pra{\jref@jnl{Phys.~Rev.~A}}%
          % Physical Review A: General Physics
\newcommand\prb{\jref@jnl{Phys.~Rev.~B}}%
          % Physical Review B: Solid State
\newcommand\prc{\jref@jnl{Phys.~Rev.~C}}%
          % Physical Review C
\newcommand\prd{\jref@jnl{Phys.~Rev.~D}}%
          % Physical Review D
\newcommand\pre{\jref@jnl{Phys.~Rev.~E}}%
          % Physical Review E
\newcommand\prl{\jref@jnl{Phys.~Rev.~Lett.}}%
          % Physical Review Letters
\newcommand\pasp{\jref@jnl{PASP}}%
          % Publications of the ASP
\newcommand\pasj{\jref@jnl{PASJ}}%
          % Publications of the ASJ
\newcommand\qjras{\jref@jnl{QJRAS}}%
          % Quarterly Journal of the RAS
\newcommand\skytel{\jref@jnl{S\&T}}%
          % Sky and Telescope
\newcommand\solphys{\jref@jnl{Sol.~Phys.}}%
          % Solar Physics
\newcommand\sovast{\jref@jnl{Soviet~Ast.}}%
          % Soviet Astronomy
\newcommand\ssr{\jref@jnl{Space~Sci.~Rev.}}%
          % Space Science Reviews
\newcommand\zap{\jref@jnl{ZAp}}%
          % Zeitschrift fuer Astrophysik
\newcommand{\znat}{Z. Naturforsch}
          % Zeitschrift fuer Naturforschung
\newcommand\nat{\jref@jnl{Nature}}%
          % Nature
\newcommand\iaucirc{\jref@jnl{IAU~Circ.}}%
          % IAU Cirulars
\newcommand\aplett{\jref@jnl{Astrophys.~Lett.}}%
          % Astrophysics Letters
\newcommand\apspr{\jref@jnl{Astrophys.~Space~Phys.~Res.}}%
          % Astrophysics Space Physics Research
\newcommand\bain{\jref@jnl{Bull.~Astron.~Inst.~Netherlands}}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{\jref@jnl{Fund.~Cosmic~Phys.}}%
          % Fundamental Cosmic Physics
\newcommand\gca{\jref@jnl{Geochim.~Cosmochim.~Acta}}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{\jref@jnl{Geophys.~Res.~Lett.}}%
          % Geophysics Research Letters
\newcommand\jcp{\jref@jnl{J.~Chem.~Phys.}}%
          % Journal of Chemical Physics
\newcommand\jcop{\jref@jnl{J.~Comp.~Phys.}}%
          % Journal of Computational Physics
\newcommand\jgr{\jref@jnl{J.~Geophys.~Res.}}%
          % Journal of Geophysics Research
\newcommand{\jkas}{Journ. Korean. Astron. Soc.}
          % Journal of the Korean Astronomical Society
\newcommand\jqsrt{\jref@jnl{J.~Quant.~Spec.~Radiat.~Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{\jref@jnl{Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{\jref@jnl{Nucl.~Phys.~A}}%
          % Nuclear Physics A
\newcommand\physrep{\jref@jnl{Phys.~Rep.}}%
          % Physics Reports
\newcommand\physscr{\jref@jnl{Phys.~Scr}}%
          % Physica Scripta
\newcommand\planss{\jref@jnl{Planet.~Space~Sci.}}%
          % Planetary Space Science
\newcommand\procspie{\jref@jnl{Proc.~SPIE}}%
          % Proceedings of the SPIE

